Stream Reasoning on Expressive Logics

Data streams occur widely in various real world applications. The research on streaming data mainly focuses on the data management, query evaluation and optimization on these data, however the work on reasoning procedures for streaming knowledge bases on both the assertional and terminological levels is very limited. Typically reasoning services on large knowledge bases are very expensive, and need to be applied continuously when the data is received as a stream. Hence new techniques for optimizing this continuous process is needed for developing efficient reasoners on streaming data. In this paper, we survey the related research on reasoning on expressive logics that can be applied to this setting, and point to further research directions in this area.

==> tex/discussion.tex <==
\section{Comparison}
\label{sec:discussion}
In this section, we compare the existing work in terms of various parameters
related to stream reasoning. The comparison is given in Table \ref{tab:comp}.
In this table, the first column lists the logic the technique is applicable to,
the second column lists the reasoning problem it is concerned with,
the third column lists whether the reasoning process is monotonic or not,
the fourth column states whether the proposed reasoning method is sound and/or complete,
and finally the last column states whether the streaming knowledge is on the
terminological and/or assertional level.


%\begin{table}
%\centering
%\begin{tabular}{ | l |l | l | l | l | }
%\hline
%& \cite{Wiener06}  & \cite{Parsia06}& \cite{Grau07} & \cite{Elgot88,Elgot99} \\
%\hline
%Logic& OWL-DL & OWL-DL& OWL-DL&Step Logic/Active Logic \\
%Reasoning Problem(s)& consistency checking & classification& classification&rule-based query answering \\
%Monotonic& Yes & Yes& No&No \\
%Sound/Complete& both & sound& sound&sound \\
%Terminological/Assertional& Assertional & Terminological& Terminological&Both \\
%Add/Delete& both & both& both&Both \\
%\hline
%\end{tabular}
%\newline
%\newline
%\caption{Comparison among existing work}
%\label{tab:comp}
%\end{table}


\begin{table}
\centering
\begin{tabular}{ | l |l | l | l | l | l|}
\hline
& Logic  & Reasoning Problem(s)& Monotonic & Sound/&Terminological/ \\
&  & &  & Complete&Assertional \\
\hline
\cite{Wiener06}& $\mathcal{SHOQ (D)}$/$\mathcal{SHIQ (D)}$ & Consistency Checking& Yes&Both & Assertional  \\
\cite{Parsia06}& $\mathcal{SHOIN (D)}$ & Classification& Yes&Sound & Terminological  \\
\cite{Grau07} & $\mathcal{SHOIQ}$ & Classification& No& Sound & Terminological  \\
\cite{Elgot88,Elgot99}& Step/Active Logic & Query Answering& No& Sound & Both  \\
\cite{\cite{Bonner96}}& Concurrent Transaction Logic & Query Answering& No& Both & Assertional  \\
\hline
\end{tabular}
\newline
\newline
\caption{Comparison among existing work}
\label{tab:comp}
\end{table}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../psi"
%%% End:


==> tex/dlres.tex <==
\section{Description Logics}
\label{sec:dl}
The stream reasoning research in Description Logics includes methods proposed
for incremental A-Box \cite{Wiener06} and T-Box \cite{Parsia06,Grau07}
reasoning. The following reasoning problem
based on an example given in \cite{Grau07} demonstrates
relevant aspects of incremental reasoning.

\newcommand{\indentruledl}{\hbox to 5mm{\hfil}}


\begin{example}\label{ex:dl}
Consider the following ontology $O^1$:


\vskip2mm
\noindent
$\indentruledl D1:$ $Cystic\_Fibrosis \equiv Fibrosis \sqcap \exists located\_In.Pancreas$\\
$\indentruledl D2:$ $Pancreatic\_Fibrosis \equiv Fibrosis \sqcap \exists Pancreatic\_Disorder$\\
$\indentruledl S1:$ $Pancreatic\_Disorder \sqsubseteq Disorder \sqcap \exists located\_In.Pancreas$\\

\noindent
The following conclusions can be drawn from  $O^1$:
\vskip2mm
\noindent
$\indentruledl C1:$ $Pancreatic\_Fibrosis \sqsubseteq Cystic\_Fibrosis$\\
$\indentruledl C2:$ $Pancreatic\_Fibrosis \sqsubseteq Disorder$\\
\vskip2mm

\noindent
$C1$ follows from $D1,$ $D2$, and $S1$. $C2$ follows from $D2$ and $S1$.
Now consider an update on the axiom $D1$ of $O^1$ which results in a modified ontology $O^2$:

\vskip2mm
\noindent
$\indentruledl D1^\prime:$ $Cystic\_Fibrosis \equiv Fibrosis \sqcap \exists located\_In.Pancreas \sqcap \\
{\hbox to 40mm{\hfil}} \exists has\_Origin.Genetic\_Origin$\\

\noindent
The conclusion $C1$ now becomes:

\vskip2mm
\noindent
$\indentruledl \neg (C1^\prime:$ $Pancreatic\_Fibrosis \sqsubseteq Cystic\_Fibrosis)$\\
\vskip2mm



\noindent
Since we know that $C1$ follows from $D1$, $D2,$ and $S1$ when any of these change we need to check if
$C1$ still hold, however since $C2$ does not depend on $D1$ we can conclude that it will still hold after the update.
%These reasoning steps can be represented as shown in Figure~\ref{fig:srextwo} in the streaming setting.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex2}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Stream Reasoning Example for Description Logics}
%\label{fig:srextwo}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex2.eps,width=75mm}}
%\caption{Stream Reasoning Example for Description Logics}
%\label{fig:srextwo}
%%\vspace*{-5mm}
%\end{figure}


The work on incremental reasoning on dynamic A-Boxes~\cite{Wiener06} investigates the process of
updating tableau completion graphs used for consistency checking incrementally.
This technique is proposed for $\mathcal{SHOQ (D)}$ and $\mathcal{SHIQ (D)}$ which
correspond to a large subset of OWL-DL. The presented algorithm for updating completion graphs
considers both addition and removal of A-Box assertions where the addition case is
straightforward due to the incremental and non-deterministic nature of the tableau algorithm.
An empirical analysis of the algorithm through an implementation in the Pellet\footnote{http://clarkparsia.com/pellet/}
reasoner is also provided.
The presented results demonstrate orders of magnitude performance improvement.

Related T-Box reasoning techniques include incrementally updating classifications of
ontologies encoded in $\mathcal{SHOIN (D)}$ which also corresponds to OWL-DL \cite{Parsia06}.
Classification is the determination for every two named classes $A$ and $B$ in an ontology
whether $A$ subsumes $B$ and vice versa. Classification involves $n^2$ subsumption tests for
$n$ named classes in the worst case. Since subsumption tests are typically very expensive, optimization
techniques for classification involves avoiding unnecessary tests and substituting
cheap tests (sound but possibly incomplete) whenever possible. The techniques proposed
for incremental reasoning includes the utilization of these optimizations to the streaming setting
where there are axiom additions and deletions.
The optimization on avoiding tests involve maintaining a subsumption hierarchy and whenever a new axiom is added
using this information to reduce the number of subsumption tests needed for the classification after the update.
This technique is independent from the reasoning algorithm used, hence it can be used for incremeantal reasoning
in other logical formalisms.
The second optimization on using cheaper tests uses the notion of model caching~\cite{Horrocks97}
(or pseudo model caching as in~\cite{Haarslev01}). The general idea is to build pseudo models
during the satisfiability checking of classes which is done prior to classification.
These models can be reused in subsumption checking. If a model of a class $A$ and a model of a class
$\neg B$ can be combined into a a single model then their conjunction is satisfiable which also
means $A$ does not subsume $B$. Hence whenever a new axiom is added to the T-Box the previously built
pseudo models can be used for incremental classification. This approach is sound but incomplete.
Since most subsumption tests are negative, it can dramatically improve the classification performance.
The empirical analysis of the mentioned techniques using the Pellet
reasoner  \cite{Parsia06} also show promising results.

The second incremental reasoning technique for T-Boxes~\cite{Grau07} also involves reusing of information
obtained from previous versions of a T-Box. The proposed method is based on the notion of a module and can be
applied to arbitrary queries against ontologies expressed in OWL-DL.
The general idea is to keep track of evidences for both subsumption and non-subsumption relationships
to be reused after an update to the ontology. For the classification of subsumptions after an update,
the axioms that each subsumption follows from is stored and if the update does not change
any of these axioms it is guaranteed that the subsumption will still hold after the update.
For determining the entailment of non-subsumtions, again an evidence can be used such as a counter model
that is constructed by tableaux-based procedures which can be reused for reasoning about non-subsumtions
after a T-Box update as also described in \cite{Parsia06}. The evaluation of the proposed methods
demonstrate substantial speed-up when compared to regular classification.

==> tex/exp.tex <==
\section{Experiments}
\label{sec:exp}
%
We analyze performance of the technique proposed using the XSB system.
In the experiments we present in this paper, we used a machine with 2.13 GHz
Intel(R) Core i3 processor and 4GB RAM.


%\color{blue}
We conducted experiments on two sets of formulas.
Figure~\ref{f:egraph1} and Figure~\ref{f:egraph2} shows the performance results of XSB and the incremental evaluation using XSB for conjunctive formulas
with respect to the number of conjuncts ($n$) and response time (in seconds) where:

$\varphi$ $=$ $\varphi_1$ $\wedge$ $\varphi_2$ $\wedge$ $\ldots$ $\wedge$ $\varphi_n$ such that:
\begin{itemize}
\item $\varphi_i = x_i \in Y_i$ (Figure~\ref{f:egraph1})
\item $\varphi_i = \exists Y_i: x_i \in Y_i$ (Figure~\ref{f:egraph2})
\end{itemize}
where $x_i$ is a first order variable and $Y_i$ is a second order variable
($n \geq 1$).


The results show that the time for evaluating a series of conjunctive formulas with the traditional methods and incremental methods
differ considerably.

\begin{figure}[t]
\centerline{\fbox{\psfig{figure=exp/expres1.ps,width=75mm}}}
\caption{Performance (secs) w.r.t.\ increasing number of atomic formulas in conjunctive formulas where $\varphi_i = x_i \in Y_i$}.
\label{f:egraph1}
%\vspace*{-5mm}
\end{figure}

\begin{figure}[t]
\centerline{\fbox{\psfig{figure=exp/expres2.ps,width=75mm}}}
\caption{Performance (secs) w.r.t.\ increasing number of atomic formulas in conjunctive formulas where $\varphi_i = \exists Y_i: x_i \in Y_i$}.
\label{f:egraph2}
%\vspace*{-5mm}
\end{figure}

There are two time components in this problem where one is the CPU time and the other is the processing time. When we consider evaluating
a series of formulas:

$\varphi_1$ , $\varphi_1$ $\wedge$ $\varphi_2$, \ldots, $\varphi_1$ $\wedge$ $\varphi_2$ $\wedge$ $\ldots$ $\wedge$ $\varphi_n$

The total time needed to evaluate this series of formulas with traditional evaluation can be computed using the following formula:

$\sum\limits_{i=1}^n C_{\phi_i} + P_{\phi_i}$

\noindent
whereas the total time needed to evaluate the series of formulas with incremental evaluation can be approximated using the following formula:

$C_{\phi_1} + \sum\limits_{i=1}^n P_{\phi_i}$

\noindent
where $\phi_i$ is $\varphi_1$ $\wedge$ $\varphi_2$ $\wedge$ $\ldots$ $\wedge$ $\varphi_i$, $C_{\phi_i}$ is the CPU time for evaluating
the logic program that represents $\phi_i$, and $P_{\phi_i}$ is the processing time for evaluating
the logic program that represents $\phi_i$.






==> tex/otherl.tex <==
\section{Rule-based and Temporal Logics}
\label{sec:other}
In this section, we will outline relevant work on rule based and temporal logics which is
mainly based on Default Logic~\cite{Reiter80}.
The main reason for this is that Default Logic can capture the dynamic nature of the reasoning process and derived
conclusions better than other rule based logical formalisms which we will describe in further detail later in this section.
The following example shows how a rule-based evaluation problem can be applied on a streaming setting.

\newcommand{\indentrule}{\hbox to 25mm{\hfil}}

\begin{example}\label{ex:reach}
Consider we have connectivity information on a set of Web pages which is updated frequently
as new pages enter or leave and a program computing reachability among these Web pages
represented by the following program:

\vskip2mm
\noindent
$\indentrule connected(w_1,w_2).$ \\
$\indentrule connected(w_2,w_3).$ \\
$\indentrule \ldots$ \\
$\indentrule \ldots$ \\
$\indentrule \ldots$ \\
\vskip2mm
\noindent
$\indentrule reachable(W,Z) \leftarrow connected(W,Z).$ \\
$\indentrule reachable(W,Z) \leftarrow reachable(W,Y), connected(Y,Z).$ \\
\vskip2mm

\noindent
%This problem can be represented as shown in Figure~\ref{fig:srex} in the streaming setting.
We need efficient procedures for maintaining the reachability information and answering queries on the program as
new data arrives and leaves. For instance we should not recompute the fact $reachable(w_1,w_2)$ in the reasoning process
after the arrival of the fact $connected(w_2,w_3)$.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex1}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex1.eps,width=75mm}}
%\caption{Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex}
%%\vspace*{-5mm}
%\end{figure}


In addition to the streaming nature of knowledge, the reasoning itself can also be considered as an
ongoing process deducing a stream of conclusions over time rather than focusing on the end results.
This adds the notion of time to the reasoning process. In~\cite{Elgot88},
Step Logic is introduced as a formalism which is used to characterize this ongoing process of
reasoning. In this setting, the reasoner starts out with an empty set of beliefs at time zero and
certain conclusions or observations may arise at discrete time steps. Hence, they can
represent streaming knowledge and conclusions. A subset of the overall knowledge base is the
focus of attention at a certain time which also adds a new dimension, namely space, to the reasoning process.
Conclusions can be drawn from the current set of beliefs and also can be retracted when additional knowledge
arrives. The inconsistencies can be dealt by tagging rules and facts based on their source such as
observation or deduction, and also by considering the time parameters of the contradictory facts
that are generated. A description of such a system is given in~\cite{Elgot91}. Efficient
reasoning techniques for such a system that reuses its previous deduction steps and
selects the relevant parts of the knowledge base for reasoning still needs to be explored.

Active Logic~\cite{Elgot99} introduced after Step logic also considers reasoning as an ongoing process
altering plans and beliefs accordingly. Similarly a uniform, lightweight language specification for
a class of temporal logics for reasoning about action and change is described in~\cite{Doherty98}.

The following example demonstrates the use of a non-monotonic reasoning problem on a streaming knowledge base.



\begin{example}\label{ex:default}
Consider the following program (terminology),

\vskip2mm
\noindent
$\indentrule flies(X) \leftarrow bird(X).$ \\
$\indentrule \neg flies(X) \leftarrow ostrich(X).$ \\
\vskip2mm

\noindent
and the streaming fact base (assertions):
%is illustrated in Figure~\ref{fig:srex3}:

\vskip2mm
\noindent
$\indentrule bird(tweety).$ \\
$\indentrule ostrich(tweety).$ \\
\vskip2mm


\noindent
Note that the fact $flies(tweety)$ is derived from the fist rule, and as new information revealing
the fact $ostrich(tweety)$ arrives $\neg flies(tweety)$ is derived which contradicts with the
previous conclusion. Since $\neg flies(tweety)$
is more recent (deduced after $flies(tweety)$ when the new information $ostrich(tweety)$ arrived to the fact base)
the previous one can be ignored which
can be implemented naturally in the streaming setting since it has a time dimension.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex3}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Non-monotonic Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex3}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex3.eps,width=75mm}}
%\caption{Non-monotonic Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex3}
%%\vspace*{-5mm}
%\end{figure}


There are several other techniques on dynamic reasoning methods for
various fragments of first order logic. Work on constraint
programming architectures \cite{Robin07} outlines the desirable
properties of such platforms which also include the solution
adaptation. The availability of this property among others is in
several constraint programming platforms is noted and a new
architecture with this property is proposed. The main solution
adaptation technique mentioned is {\it Justification Based Truth
Maintenance} where each solution is kept with the indexes of the
rules that it is derived from which is similar to the incremental
techniques we outlined for Description Logics. The work on solving
database integrity constraints \cite{Henning06} aims for producing
simplified incremental checks for each database update.

There is also work on programming paradigms such as {\it Finite Differencing} \cite{Paige90}
which is an old mathematical idea that can speed up computation by replacing repeated costly calculations
by more efficient counterparts. In addition to this, Dynamic Logic \cite{Harel84} is proposed as a formal
system for reasoning about programs. The name {\it Dynamic Logic} emphasizes the principal feature
distinguishing it from classical predicate logic. In the latter, the truth is static.
In Dynamic Logic, there are explicit syntactic constructs called programs whose main role is to change
the values of variables, thereby changing the truth values of programs.


Furthermore, there is work on belief revision \cite{Darwiche96,Eijck08} which is the process of changing beliefs to
take into account new pieces of information, where one method is the use of Default Logic explained in this paper.
Work on interpreting and summarizing (i.e. compressing) streaming factual data
is also relevant to stream reasoning which involves techniques form
logical formalisms such as Inductive Logic Programming \cite{Muggleton94}.

After the introduction of stream reasoning \cite{SR2009intro} new techniques on various formalisms emerged. One of them
is Stream reasoning on Answer Set programming (ASP) \cite{Gebser12} which provides
language constructs and modeling techniques for reasoning on time-decaying logic programs. The stream reasoning
capability is incorporated to the logic programming language with additional ASP constructs for the emergence and expiration of program parts.

Stream reasoning on a temporal rule-based formalism called LARS \cite{BeckDE15} with semantics similar to Answer Set Programming is also a recent work in the area. The work presented provides an incremental answer update algorithm on a fragment of LARS programs based on stream stratification which extends techniques from truth maintenance systems.



==> tex/relwork.tex <==
\section{Related Work}
\label{sec:relwork}

In this section, we provide the related work on stream reasoning with regards to Description Logics and Rule-based and Temporal Logics.

\subsection{Description Logics}
\label{sec:dl}
The stream reasoning research in Description Logics includes methods proposed
for incremental A-Box \cite{Wiener06} and T-Box \cite{Parsia06,Grau07}
reasoning. The following reasoning problem
based on an example given in \cite{Grau07} demonstrates
relevant aspects of incremental reasoning.

\newcommand{\indentruledl}{\hbox to 5mm{\hfil}}


\begin{example}\label{ex:dl}
Consider the following ontology $O^1$:


\vskip2mm
\noindent
$\indentruledl D1:$ $Cystic\_Fibrosis \equiv Fibrosis \sqcap \exists located\_In.Pancreas$\\
$\indentruledl D2:$ $Pancreatic\_Fibrosis \equiv Fibrosis \sqcap \exists Pancreatic\_Disorder$\\
$\indentruledl S1:$ $Pancreatic\_Disorder \sqsubseteq Disorder \sqcap \exists located\_In.Pancreas$\\

\noindent
The following conclusions can be drawn from  $O^1$:
\vskip2mm
\noindent
$\indentruledl C1:$ $Pancreatic\_Fibrosis \sqsubseteq Cystic\_Fibrosis$\\
$\indentruledl C2:$ $Pancreatic\_Fibrosis \sqsubseteq Disorder$\\
\vskip2mm

\noindent
$C1$ follows from $D1,$ $D2$, and $S1$. $C2$ follows from $D2$ and $S1$.
Now consider an update on the axiom $D1$ of $O^1$ which results in a modified ontology $O^2$:

\vskip2mm
\noindent
$\indentruledl D1^\prime:$ $Cystic\_Fibrosis \equiv Fibrosis \sqcap \exists located\_In.Pancreas \sqcap \\
{\hbox to 40mm{\hfil}} \exists has\_Origin.Genetic\_Origin$\\

\noindent
The conclusion $C1$ now becomes:

\vskip2mm
\noindent
$\indentruledl \neg (C1^\prime:$ $Pancreatic\_Fibrosis \sqsubseteq Cystic\_Fibrosis)$\\
\vskip2mm



\noindent
Since we know that $C1$ follows from $D1$, $D2,$ and $S1$ when any of these change we need to check if
$C1$ still hold, however since $C2$ does not depend on $D1$ we can conclude that it will still hold after the update.
%These reasoning steps can be represented as shown in Figure~\ref{fig:srextwo} in the streaming setting.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex2}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Stream Reasoning Example for Description Logics}
%\label{fig:srextwo}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex2.eps,width=75mm}}
%\caption{Stream Reasoning Example for Description Logics}
%\label{fig:srextwo}
%%\vspace*{-5mm}
%\end{figure}


The work on incremental reasoning on dynamic A-Boxes~\cite{Wiener06} investigates the process of
updating tableau completion graphs used for consistency checking incrementally.
This technique is proposed for $\mathcal{SHOQ (D)}$ and $\mathcal{SHIQ (D)}$ which
correspond to a large subset of OWL-DL. The presented algorithm for updating completion graphs
considers both addition and removal of A-Box assertions where the addition case is
straightforward due to the incremental and non-deterministic nature of the tableau algorithm.
An empirical analysis of the algorithm through an implementation in the Pellet\footnote{http://clarkparsia.com/pellet/}
reasoner is also provided.
The presented results demonstrate orders of magnitude performance improvement.

Related T-Box reasoning techniques include incrementally updating classifications of
ontologies encoded in $\mathcal{SHOIN (D)}$ which also corresponds to OWL-DL \cite{Parsia06}.
Classification is the determination for every two named classes $A$ and $B$ in an ontology
whether $A$ subsumes $B$ and vice versa. Classification involves $n^2$ subsumption tests for
$n$ named classes in the worst case. Since subsumption tests are typically very expensive, optimization
techniques for classification involves avoiding unnecessary tests and substituting
cheap tests (sound but possibly incomplete) whenever possible. The techniques proposed
for incremental reasoning includes the utilization of these optimizations to the streaming setting
where there are axiom additions and deletions.
The optimization on avoiding tests involve maintaining a subsumption hierarchy and whenever a new axiom is added
using this information to reduce the number of subsumption tests needed for the classification after the update.
This technique is independent from the reasoning algorithm used, hence it can be used for incremeantal reasoning
in other logical formalisms.
The second optimization on using cheaper tests uses the notion of model caching~\cite{Horrocks97}
(or pseudo model caching as in~\cite{Haarslev01}). The general idea is to build pseudo models
during the satisfiability checking of classes which is done prior to classification.
These models can be reused in subsumption checking. If a model of a class $A$ and a model of a class
$\neg B$ can be combined into a a single model then their conjunction is satisfiable which also
means $A$ does not subsume $B$. Hence whenever a new axiom is added to the T-Box the previously built
pseudo models can be used for incremental classification. This approach is sound but incomplete.
Since most subsumption tests are negative, it can dramatically improve the classification performance.
The empirical analysis of the mentioned techniques using the Pellet
reasoner  \cite{Parsia06} also show promising results.

The second incremental reasoning technique for T-Boxes~\cite{Grau07} also involves reusing of information
obtained from previous versions of a T-Box. The proposed method is based on the notion of a module and can be
applied to arbitrary queries against ontologies expressed in OWL-DL.
The general idea is to keep track of evidences for both subsumption and non-subsumption relationships
to be reused after an update to the ontology. For the classification of subsumptions after an update,
the axioms that each subsumption follows from is stored and if the update does not change
any of these axioms it is guaranteed that the subsumption will still hold after the update.
For determining the entailment of non-subsumtions, again an evidence can be used such as a counter model
that is constructed by tableaux-based procedures which can be reused for reasoning about non-subsumtions
after a T-Box update as also described in \cite{Parsia06}. The evaluation of the proposed methods
demonstrate substantial speed-up when compared to regular classification.

\subsection{Rule-based and Temporal Logics}
\label{sec:other}
In this section, we will outline relevant work on rule based and temporal logics which is
mainly based on Default Logic~\cite{Reiter80}.
The main reason for this is that Default Logic can capture the dynamic nature of the reasoning process and derived
conclusions better than other rule based logical formalisms which we will describe in further detail later in this section.
The following example shows how a rule-based evaluation problem can be applied on a streaming setting.

\newcommand{\indentrule}{\hbox to 25mm{\hfil}}

\begin{example}\label{ex:reach}
Consider we have connectivity information on a set of Web pages which is updated frequently
as new pages enter or leave and a program computing reachability among these Web pages
represented by the following program:

\vskip2mm
\noindent
$\indentrule connected(w_1,w_2).$ \\
$\indentrule connected(w_2,w_3).$ \\
$\indentrule \ldots$ \\
$\indentrule \ldots$ \\
$\indentrule \ldots$ \\
\vskip2mm
\noindent
$\indentrule reachable(W,Z) \leftarrow connected(W,Z).$ \\
$\indentrule reachable(W,Z) \leftarrow reachable(W,Y), connected(Y,Z).$ \\
\vskip2mm

\noindent
%This problem can be represented as shown in Figure~\ref{fig:srex} in the streaming setting.
We need efficient procedures for maintaining the reachability information and answering queries on the program as
new data arrives and leaves. For instance we should not recompute the fact $reachable(w_1,w_2)$ in the reasoning process
after the arrival of the fact $connected(w_2,w_3)$.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex1}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex1.eps,width=75mm}}
%\caption{Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex}
%%\vspace*{-5mm}
%\end{figure}


In addition to the streaming nature of knowledge, the reasoning itself can also be considered as an
ongoing process deducing a stream of conclusions over time rather than focusing on the end results.
This adds the notion of time to the reasoning process. In~\cite{Elgot88},
Step Logic is introduced as a formalism which is used to characterize this ongoing process of
reasoning. In this setting, the reasoner starts out with an empty set of beliefs at time zero and
certain conclusions or observations may arise at discrete time steps. Hence, they can
represent streaming knowledge and conclusions. A subset of the overall knowledge base is the
focus of attention at a certain time which also adds a new dimension, namely space, to the reasoning process.
Conclusions can be drawn from the current set of beliefs and also can be retracted when additional knowledge
arrives. The inconsistencies can be dealt by tagging rules and facts based on their source such as
observation or deduction, and also by considering the time parameters of the contradictory facts
that are generated. A description of such a system is given in~\cite{Elgot91}. Efficient
reasoning techniques for such a system that reuses its previous deduction steps and
selects the relevant parts of the knowledge base for reasoning still needs to be explored.

Active Logic~\cite{Elgot99} introduced after Step logic also considers reasoning as an ongoing process
altering plans and beliefs accordingly. Similarly a uniform, lightweight language specification for
a class of temporal logics for reasoning about action and change is described in~\cite{Doherty98}.

The following example demonstrates the use of a non-monotonic reasoning problem on a streaming knowledge base.



\begin{example}\label{ex:default}
Consider the following program (terminology),

\vskip2mm
\noindent
$\indentrule flies(X) \leftarrow bird(X).$ \\
$\indentrule \neg flies(X) \leftarrow ostrich(X).$ \\
\vskip2mm

\noindent
and the streaming fact base (assertions):
%is illustrated in Figure~\ref{fig:srex3}:

\vskip2mm
\noindent
$\indentrule bird(tweety).$ \\
$\indentrule ostrich(tweety).$ \\
\vskip2mm


\noindent
Note that the fact $flies(tweety)$ is derived from the fist rule, and as new information revealing
the fact $ostrich(tweety)$ arrives $\neg flies(tweety)$ is derived which contradicts with the
previous conclusion. Since $\neg flies(tweety)$
is more recent (deduced after $flies(tweety)$ when the new information $ostrich(tweety)$ arrived to the fact base)
the previous one can be ignored which
can be implemented naturally in the streaming setting since it has a time dimension.
\end{example}


%\begin{figure}[t]
%%\sidecaption
%\includegraphics[scale=.70]{figures/srex3}
%%
%% If no graphics program available, insert a blank space i.e. use
%%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%%
%\caption{Non-monotonic Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex3}       % Give a unique label
%\end{figure}

%\begin{figure}[t]
%\centerline{\psfig{figure=figures/srex3.eps,width=75mm}}
%\caption{Non-monotonic Stream Reasoning Example for Rule-based Logics}
%\label{fig:srex3}
%%\vspace*{-5mm}
%\end{figure}


There are several other techniques on dynamic reasoning methods for
various fragments of first order logic. Work on constraint
programming architectures \cite{Robin07} outlines the desirable
properties of such platforms which also include the solution
adaptation. The availability of this property among others is in
several constraint programming platforms is noted and a new
architecture with this property is proposed. The main solution
adaptation technique mentioned is {\it Justification Based Truth
Maintenance} where each solution is kept with the indexes of the
rules that it is derived from which is similar to the incremental
techniques we outlined for Description Logics. The work on solving
database integrity constraints \cite{Henning06} aims for producing
simplified incremental checks for each database update.

There is also work on programming paradigms such as {\it Finite Differencing} \cite{Paige90}
which is an old mathematical idea that can speed up computation by replacing repeated costly calculations
by more efficient counterparts. In addition to this, Dynamic Logic \cite{Harel84} is proposed as a formal
system for reasoning about programs. The name {\it Dynamic Logic} emphasizes the principal feature
distinguishing it from classical predicate logic. In the latter, the truth is static.
In Dynamic Logic, there are explicit syntactic constructs called programs whose main role is to change
the values of variables, thereby changing the truth values of programs.


Furthermore, there is work on belief revision \cite{Darwiche96,Eijck08} which is the process of changing beliefs to
take into account new pieces of information, where one method is the use of Default Logic explained in this paper.
Work on interpreting and summarizing (i.e. compressing) streaming factual data
is also relevant to stream reasoning which involves techniques form
logical formalisms such as Inductive Logic Programming \cite{Muggleton94}.





==> tex/resmonadic.tex <==

\def\dcv{\mbox{\rm Datalog$^{\mathrm{cv}}$}}
\def\binarytree{$(0+1)^*$ $=$ $\{\epsilon,$ $0,$ $1,$ $00,$ $01,$ $10,$ $11,$ $000,$ $...\}$}
\def\xbar{\overline{x}}
\def\ybar{\overline{y}}
\def\zbar{\overline{z}}
\def\obar{\overline{o}}

\def\Node{\mathsf{Node}}
\def\Start{\mathsf{Start}}
\def\Final{\mathsf{Final}}
\def\Transition{\mathsf{Trans}}
\def\TransClos{\mathsf{TransClos}}
\def\ZorO{\mathsf{Zero\_or\_One}}

%\newcommand{\indentrule}{\hbox to 25mm{\hfil}}

\section{Stream Reasoning on Monadic Second-order Logics}
\label{sec:strmonadic}

Monadic second-order logics provide means to specify regular
properties of systems in a succinct way. In addition, these logics are
decidable by the virtue of the connection to automata theory \cite{Buchi,Rabin}.
% This connection has been known since the 1960's.
However, only recently tools based on these ideas---in particular the
MONA system \cite{Klarlund}---have been developed and shown to be
efficient enough for practical applications \cite{Henriksen}.
%One of the main advances toward
%improving the efficiency of such tools has been the introduction of
%binary decision diagrams (BDD) \cite{Bryant92} and other state-space
%compression techniques for representing the automaton's transitions in
%a compact way.

% Recently, the MONA reasoner has been used as the basis for reasoning
% in the description logic ${\cal ALC}$ \cite{Karabaev}: ${\cal ALC}$
% concepts have been mapped to equisatisfiable WS1S or WS2S formul\ae.
% Similar techniques have been designed for more expressive description
% logics as well.

%\begin{figure}
%\scalebox{0.7}{ \input{exp1.pdf} }
%\caption{Relation between join ordering and formula rewriting}
%\label{f:jorder}
%\end{figure}



% The experimental results presented in that paper have shown that the
% MONA system can be used for testing concept satisfiability.
However, for reasoning in large theories consisting of relatively
simple constraints, such as theories capturing UML class diagrams or
database schemata, the MONA system runs into a~serious state-space
explosion problem---the size of the automaton capturing the (language
of) models for a given formula quickly exceeded the space available in
most computers.
%
% This was contrasted with the theoretically sub-optimal tableaux
% methods that in practice are able to handle much larger inputs
% \cite{racer,fact}.
%
The problem can be traced to the \emph{automata product}
operation that is used to translate conjunctions in the original
formul\ae\ rather than to the theoretically more problematic
projection/determinization operations
needed to handle quantifier alternations.
% ; indeed only single quantifier
% alternation is needed in the (translations of) ${\cal ALC}$
% implication problems.

A technique that combats this problem is provided \cite{Unel07} which is based on techniques
developed for query evaluation in deductive databases, in particular
on the \emph{Magic Set transformation} (Beeri and Naqvi et al. 1991)
%\cite{Beeri2}
and the \emph{SLG resolution}, a top-down resolution-based approach augmented with
memoization \cite{Warren95,Warren93}. The work establishes the connection
between the auto\-mata-based decision procedures for WS1S (and,
analogously, for WS2S) and query evaluation in Complex-value Datalog
(\dcv) \cite{Abiteoul}.  The approach is based on
representing automata using nested relations and on defining the
necessary automata-theoretic operations using \dcv\ programs. This
reduces the satisfiability of a WSnS formula to posing a closed \dcv\ goal over a \dcv\ program
representing impicitly the final automaton.
%
This observation combined with powerful program execution techniques
developed for deductive databases, such as the Magic Set rewriting and
SLG resolution, in many cases limit the explored state space to elements needed to
show non-emptiness of the automaton and, in turn, satisfiability of
the corresponding formula.

This approach can be extended to a stream reasoning solution on monadic second-order logics where the problem can be defined as follows.
Given an ordered set of formulas $\{\varphi_1,$
$\varphi_2,$ $\ldots,$ $\varphi_n\}$ determine if the conjunction of the formulas at each step is satisfiable without generating the whole
automaton representing the conjunction. This problem is solved by generating a set of logic programs representing the conjunction of formulas
at each step where the query representing the satisfiability of a formula is evaluated using incremental evaluation techniques provided
for logic programs \cite{Swift10}. This method can be used for reasoning on a series of formulas on large theories, such as
those corresponding to constraints used in database schemata or UML diagrams. 

==> tex/srsystems.tex <==
\section{Towards Stream Reasoning Systems}
\label{sec:srsystems}
In recent years research towards stream reasoning systems provided architectures and results.
Firstly, a stream reasoning architecture for handling different complexity levels by the notion of cascading reasoners
was proposed \cite{Heiner10}. The architecture is designed to provide a wide array of reasoning capabilities from
raw stream processing to complex Description Logic reasoning.

ETALIS - a system that performs stream reasoning on top of Complex Event Processing (CEP) is implemented later
which provide real-time specification and monitoring of changes \cite{ARFS2012}. The system improves CEP by performing reasoning on streams combined with background knowledge on-the-fly using a deductive rule-based paradigm.
Event-driven processing is included which enables the system to derive a complex event at the moment it occurs.
An extension of ETALIS that accepts RDFS ontologies as background knowledge which are converted to Prolog programs
is also described. The system is implemented in Prolog and has been used in research projects.

There is also a system developed in Haskell using plausible Description Logic Programs
where the main components are description logic, plausible logic and functional programming \cite{Groza12}.
The proposed system aims handling theoretically infinite and heterogenous data streams by lazy evaluation
which is characterized as a step towards building real-time stream reasoners.

Recently, a technique was proposed for checking the satisfiability of Monadic second-order formulas incrementally
which can be used for reasoning on a series of formulas on large theories, such as
those corresponding to rapidly changing constraints encoded with expressive logics \cite{Unel2015}. The method
is implemented using logic programming which is an application of incremental reasoning over 
a very expressive logic. 
